Bolocam Survey for 1.1 mm Dust Continuum Emission in the c2d Legacy Clouds. I. Perseus

We have completed a 1.1 mm continuum survey of 7.5 sq deg of the Perseus Molecular Cloud using Bolocam at the Caltech Submillimeter Observatory. This represents the largest millimeter or submillimeter continuum map of Perseus to date. Our map covers more than 30,000 31" (FWHM) resolution elements to a 1 sigma RMS of 15 mJy/beam. We detect a total of 122 cores above a 5 sigma point source mass detection limit of 0.18 M_sun, assuming a dust temperature of 10 K, 60 of which are new millimeter or submillimeter detections. The 1.1 mm mass function is consistent with a broken power law of slope -1.3 (0.5 M_sun<M<2.5 M_sun) and -2.6 (M>2.5 M_sun), similar to the local initial mass function slope. No more than 5% of the total cloud mass is contained in discrete 1.1 mm cores, which account for a total mass of 285 M_sun. We suggest an extinction threshold for millimeter cores of Av~5 mag, based on our calculation of the probability of finding a 1.1 mm core as a function of Av. Much of the cloud is devoid of compact millimeter emission; despite the significantly greater area covered compared to previous surveys, only 5-10 of the newly identified sources lie outside previously observed areas. The two-point correlation function confirms that dense cores in the cloud are highly structured, with significant clustering on scales as large as 2e5 AU. These 1.1 mm results, especially when combined with recently acquired c2d Spitzer Legacy data, will provide a census of dense cores and protostars in Perseus and improve our understanding of the earliest stages of star formation in molecular clouds.

==> tab1.tex <==
\ProvidesFile{tab1.tex}
\begin{deluxetable}{lcccccc}
\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{Source IDs, positions, and peak flux density \label{srctab}}
\tablehead{ \colhead{ID} & \colhead{RA (2000)} & \colhead{Dec (2000)} & \colhead{Peak} &  \colhead{S/N}  & \colhead{Other Names} & \colhead{MIPS $24\micron$ Source?}  \\ 
\colhead{} & \colhead{($h ~~m ~~s$)} & \colhead{($\degr~~ \arcmin~~ \arcsec$)} & \colhead{(mJy/beam)} &  \colhead{}  & \colhead{} & \colhead{}  }

\startdata

Bolo 1  &  03 25 07.8 &  +30 24 21.6  &  109 (16)  &  6.1  &    &  N   \\
Bolo 2  &  03 25 09.5 &  +30 23 51.3  &  121 (16)  &  8.7  &    &  N   \\
Bolo 3  &  03 25 10.2 &  +30 44 43.4  &  125 (17)  &  6.6  &    &  N   \\
Bolo 4  &  03 25 17.0 &  +30 18 53.2  &  149 (17)  &  7.2  &    &  N   \\
Bolo 5  &  03 25 22.2 &  +30 45 09.3  &  727 (18)  &  42.0  & \object[IRAS 03222+3034]{L 1448-IRS2} (1)   &  Y   \\
Bolo 6  &  03 25 26.5 &  +30 21 50.0  &  143 (19)  &  5.9  &    &  N   \\
Bolo 7  &  03 25 35.4 &  +30 13 06.2  &  126 (17)  &  6.0  &    &  N   \\
Bolo 8  &  03 25 35.9 &  +30 45 17.2  &  2241 (19)  &  128  &  \object[LDN 1448N]{L 1448-N} (2)  &  Y   \\
Bolo 9  &  03 25 37.2 &  +30 09 55.4  &  113 (16)  &  5.7  &    &  N   \\
Bolo 10  &  03 25 38.4 &  +30 43 58.0  &  980 (20)  &  45.2  & \object[LDN 1448C]{L 1448-C} (2)   &  Y   \\
Bolo 11  &  03 25 46.0 &  +30 44 10.3  &  240 (20)  &  8.4  &   &  Y   \\
Bolo 12  &  03 25 47.5 &  +30 12 25.9  &  118 (18)  &  5.1  &    &  N   \\
Bolo 13  &  03 25 48.8 &  +30 42 24.1  &  407 (19)  &  19.0  &  H32 (3)   & N   \\
Bolo 14  &  03 25 50.6 &  +30 42 01.4  &  342 (19)  &  17.9  &  H33 (3)  &  N   \\
Bolo 15  &  03 25 55.1 &  +30 41 25.8  &  188 (17)  &  6.4  &    &  N   \\
Bolo 16  &  03 25 56.2 &  +30 40 41.1  &  154 (17)  &  6.3  &    &  N   \\
Bolo 17  &  03 25 58.4 &  +30 37 13.4  &  122 (15)  &  6.7  &    &  N   \\
Bolo 18  &  03 26 36.9 &  +30 15 23.0  &  225 (15)  &  14.9  &  \object{IRAS 03235+3004}; H80 (3)  &  Y   \\
Bolo 19  &  03 27 02.0 &  +30 15 07.9  &  115 (14)  &  7.3  &    &  N   \\
Bolo 20  &  03 27 28.8 &  +30 15 02.1  &  114 (16)  &  5.9  &    &  N   \\
Bolo 21  &  03 27 37.5 &  +30 13 53.4  &  164 (17)  &  9.0  &  H39 (3)  &  Y   \\
Bolo 22  &  03 27 39.3 &  +30 12 52.9  &  317 (18)  &  16.3  & \object[IRAS 03245+3002]{RNO 15-FIR} (4) &  Y   \\
Bolo 23  &  03 27 41.7 &  +30 12 24.1  &  283 (18)  &  12.8  & H36 (3)   &  Y   \\
Bolo 24  &  03 27 47.9 &  +30 12 02.1  &  220 (19)  &  11.2  & \object[IRAS 03247+3001]{L 1455-IRS2} (5); H37 (3) &  Y   \\
Bolo 25  &  03 28 32.1 &  +31 11 08.8  &  106 (16)  &  6.7  & H74 (3)  &  N/A   \\
Bolo 26  &  03 28 32.4 &  +31 04 42.9  &  117 (14)  &  7.6  &    &  N/A   \\
Bolo 27  &  03 28 33.3 &  +30 19 35.0  &  155 (16)  &  6.4  &    &  Y   \\
Bolo 28  &  03 28 34.0 &  +31 07 01.2  &  137 (14)  &  9.7  &  H69 (3) &  N/A   \\
Bolo 29  &  03 28 36.2 &  +31 13 26.4  &  267 (19)  &  17.1  &  \object[IRAS 03255+3103]{NGC 1333-IRAS 1} (6); SK6 (7) &  N/A (IRAS)   \\
Bolo 30  &  03 28 39.0 &  +31 05 59.2  &  189 (15)  &  11.3  &  \object[\[LMG94\] Per 3]{in Per3} (8); H71 (4) &  N/A   \\
Bolo 31  &  03 28 39.9 &  +31 17 56.7  &  385 (19)  &  20.1  &  \object[\[JCC87\] IRAS 5]{NGC 1333-IRAS 5} (6) &  N/A (IRAS)   \\
Bolo 32  &  03 28 41.7 &  +30 31 13.0  &  144 (15)  &  6.4  &  \object{RNO 17}  &  Y   \\
Bolo 33  &  03 28 42.6 &  +31 06 12.2  &  173 (14)  &  9.6  &  \object[\[LMG94\] Per 3]{in Per 3} (8); H75 (3)  &  N/A   \\
Bolo 34  &  03 28 45.9 &  +31 15 19.8  &  150 (20)  &  6.2  &    &  N/A   \\
Bolo 35  &  03 28 48.4 &  +31 16 01.9  &  130 (20)  &  5.9  &    &  N/A   \\
Bolo 36  &  03 28 48.7 &  +30 43 24.6  &  127 (14)  &  6.3  &    &  Y   \\
Bolo 37  &  03 28 52.1 &  +31 18 07.9  &  160 (20)  &  7.4  &  \object{ASR 40}  &  N/A   \\
Bolo 38  &  03 28 55.3 &  +31 14 32.2  &  1220 (20)  &  59.4  &  \object[IRAS 03258+3104]{NGC 1333-IRAS 2} (6,9)  &  N/A (IRAS)   \\
Bolo 39  &  03 28 55.3 &  +31 19 17.7  &  210 (20)  &  9.7  &  \object{ASR 64}; H68 (3) &  N/A   \\
Bolo 40  &  03 29 00.0 &  +31 21 37.8  &  685 (17)  &  34.2  &  \object[\[SK2001\] 31]{SK31} (7) &  N/A   \\
Bolo 41  &  03 29 00.6 &  +31 11 58.9  &  190 (19)  &  10.7  &  \object[\[SK2001\] 1]{SK1} (7) &  N/A   \\
Bolo 42  &  03 29 01.3 &  +31 20 33.0  &  1079 (18)  &  58.8  &  \object[ASR 114]{NGC 1333-IRAS 6} (6); SK24 (7)  &  N/A (IRAS)  \\
Bolo 43  &  03 29 02.6 &  +31 15 56.8  &  2160 (20)  &  103  &  \object[\[SVS76\] NGC 1333 13A]{SVS 13} (9) &  N/A   \\
Bolo 44  &  03 29 04.5 &  +31 18 42.1  &  270 (20)  &  13.7  &    &  N/A   \\
Bolo 45  &  03 29 07.7 &  +31 17 16.8  &  460 (20)  &  21.8  &  Cor 1 (9); SK17/18 (7)   &  N/A   \\
Bolo 46  &  03 29 08.3 &  +31 15 11.1  &  740 (20)  &  28.6  & \object[\[SK2001\] 16]{SK16} (7)  &  N/A   \\
Bolo 47  &  03 29 08.9 &  +31 21 43.5  &  612 (18)  &  30.9  & \object[\[SK2001\] 28]{SK28} (7)   &  N/A (IRAS)  \\
Bolo 48  &  03 29 10.9 &  +31 13 26.4  &  5180 (20)  &  264  & \object[\[JCC87\] IRAS 4]{NGC 1333-IRAS 4}  (6,10) &  N/A (IRAS)  \\
Bolo 49  &  03 29 11.3 &  +31 18 24.8  &  840 (20)  &  40.6  & \object[\[JCC87\] IRAS 7]{NGC 1333-IRAS 7} (6,9)  &  N/A (IRAS)  \\
Bolo 50  &  03 29 14.5 &  +31 20 30.1  &  310 (20)  &  14.2  &  \object[\[SK2001\] 22]{SK22} (7) &  N/A   \\
Bolo 51  &  03 29 17.0 &  +31 12 25.9  &  423 (19)  &  16.4  &  H59 (3) &  N/A   \\
Bolo 52  &  03 29 17.1 &  +31 27 38.8  &  269 (18)  &  13.7  &  \object[\[LMG94\] Per 4]{in Per 4} (8); H61 (3)  &  N/A   \\
Bolo 53  &  03 29 18.2 &  +31 25 17.0  &  336 (19)  &  16.7  &  \object[\[SK2001\] 33]{SK33} (7) &  N/A (IRAS)  \\
Bolo 54  &  03 29 19.1 &  +31 23 26.5  &  330 (19)  &  16.7  &  \object[\[SK2001\] 32]{SK32} (7) &  N/A   \\
Bolo 55  &  03 29 19.4 &  +31 11 36.6  &  184 (17)  &  9.8  &  \object{ASR 129}; H72 (3)  &   N/A   \\
Bolo 56  &  03 29 22.4 &  +31 36 24.4  &  102 (14)  &  6.8  &  H91 (3) &   N/A   \\
Bolo 57  &  03 29 22.9 &  +31 33 16.5  &  224 (16)  &  16.2  &  \object[\[LMG94\] Per 4]{in Per 4} (8); H58 (3) &  N/A (IRAS)  \\
Bolo 58  &  03 29 25.7 &  +31 28 16.3  &  273 (17)  &  14.0  &  H64 (3) &  N/A   \\
Bolo 59  &  03 29 51.5 &  +31 39 12.9  &  249 (14)  &  19.3  &  \object[\[LMG94\] Per 5]{Per 5} (8)  &  N/A (IRAS)  \\
Bolo 60  &  03 30 14.9 &  +30 23 36.9  &  125 (15)  &  8.3  & \object[IRAS 03271+3013]{IRAS 03271} (11); H15 (3); Per 6 (8)  &  Y   \\
Bolo 61  &  03 30 24.0 &  +30 27 38.5  &  106 (17)  &  5.1  &    &  N   \\
Bolo 62  &  03 30 32.0 &  +30 26 18.6  &  199 (17)  &  11.1  &    &  Y   \\
Bolo 63  &  03 30 45.5 &  +30 52 34.3  &  141 (14)  &  10.2  &    &  N/A (IRAS)  \\
Bolo 64  &  03 30 50.4 &  +30 49 17.4  &  86 (14)  &  6.4  &    &  N/A   \\
Bolo 65  &  03 31 20.0 &  +30 45 30.2  &  522 (17)  &  31.7  &  \object[IRAS 03282+3035]{IRAS 03282} (11); H77 (3)  &  N/A (IRAS)   \\
Bolo 66  &  03 32 17.3 &  +30 49 44.0  &  1068 (15)  &  73.5  & \object{IRAS 03292+3039}; H76 (3)   &  Y   \\
Bolo 67  &  03 32 26.9 &  +30 59 11.0  &  165 (19)  &  8.8  & H89 (3)   &  N   \\
Bolo 68  &  03 32 28.1 &  +31 02 17.5  &  110 (18)  &  6.6  &    &  Y   \\
Bolo 69  &  03 32 39.3 &  +30 57 28.8  &  155 (16)  &  5.7  &    &  N   \\
Bolo 70  &  03 32 44.0 &  +31 00 00.0  &  238 (17)  &  11.1  &  \object[\[LMG94\] Per 7]{in Per 7} (8)  &  N   \\
Bolo 71  &  03 32 51.2 &  +31 01 47.6  &  180 (20)  &  7.3  &    &  N   \\
Bolo 72  &  03 32 57.0 &  +31 03 20.8  &  240 (20)  &  9.4  &    &  N   \\
Bolo 73  &  03 33 00.0 &  +31 20 43.8  &  178 (16)  &  8.8  &  \object[\[LMG94\] Per 9]{in Per 9} (8) &  N   \\
Bolo 74  &  03 33 01.9 &  +31 04 31.8  &  260 (20)  &  9.3  &  H5 (3)  &  N   \\
Bolo 75  &  03 33 04.4 &  +31 04 58.8  &  260 (20)  &  9.7  &  H8 (3)  &  N   \\
Bolo 76  &  03 33 11.4 &  +31 21 30.9  &  116 (16)  &  6.5  &  \object[\[LMG94\] Per 9]{in Per 9} (8)  &  N \\
Bolo 77  &  03 33 11.4 &  +31 17 24.0  &  110 (19)  &  5.0  &    &  N   \\
Bolo 78  &  03 33 13.2 &  +31 19 50.1  &  262 (16)  &  16.3  &  \object[\[LMG94\] Per 9]{in Per 9} (8); H82 (3)  &  Y   \\
Bolo 79  &  03 33 15.0 &  +31 07 01.9  &  605 (19)  &  30.0  &  \object[\[HKM99\] B1-d]{B1-d} (12) &  Y   \\
Bolo 80  &  03 33 17.8 &  +31 09 29.8  &  1080 (20)  &  53.2  & \object[\[HKM99\] B1-c]{B1-c} (12) &  Y   \\
Bolo 81  &  03 33 20.5 &  +31 07 37.2  &  1220 (20)  &  59.9  & \object[\[HKM99\] B1-b]{B1-b} (12)  &  Y   \\
Bolo 82  &  03 33 25.1 &  +31 05 34.8  &  147 (17)  &  7.1  &   &  N   \\
Bolo 83  &  03 33 25.4 &  +31 20 07.4  &  165 (17)  &  7.2  &  \object[\[LMG94\] Per 9]{in Per 9} (8)  &  N   \\
Bolo 84  &  03 33 26.8 &  +31 06 49.6  &  190 (20)  &  7.0  &  H10 (3) &  Y   \\
Bolo 85  &  03 33 32.1 &  +31 20 03.8  &  155 (17)  &  6.9  &  \object[\[LMG94\] Per 9]{in Per 9} (8)  &  N   \\
Bolo 86  &  03 33 51.1 &  +31 12 36.7  &  131 (18)  &  5.2  &    &  Y   \\
Bolo 87  &  03 35 21.6 &  +31 06 55.4  &  99 (14)  &  5.9  &    &  N   \\
Bolo 88  &  03 40 14.5 &  +32 01 29.6  &  162 (17)  &  6.7  &    &  N   \\
Bolo 89  &  03 40 49.3 &  +31 48 34.5  &  151 (16)  &  8.1  &    &  Y   \\
Bolo 90  &  03 41 09.0 &  +31 44 33.0  &  139 (15)  &  8.0  &    &  Y   \\
Bolo 91  &  03 41 19.7 &  +31 47 28.3  &  106 (15)  &  6.5  &    &  N   \\
Bolo 92  &  03 41 40.0 &  +31 58 04.8  &  94 (14)  &  6.4  &    &  N   \\
Bolo 93  &  03 41 45.1 &  +31 48 09.7  &  118 (16)  &  6.3  &    &  N   \\
Bolo 94  &  03 41 45.8 &  +31 57 21.6  &  132 (14)  &  7.3  &    &  N   \\
Bolo 95  &  03 42 20.6 &  +31 44 49.2  &  108 (14)  &  6.2  &    &  Y   \\
Bolo 96  &  03 42 47.1 &  +31 58 40.8  &  148 (16)  &  7.1  &    &  N   \\
Bolo 97  &  03 42 52.3 &  +31 58 12.3  &  149 (17)  &  6.0  &    &  Y   \\
Bolo 98  &  03 42 57.3 &  +31 57 49.3  &  134 (18)  &  6.0  &    &  Y   \\
Bolo 99  &  03 43 38.3 &  +32 03 08.6  &  164 (13)  &  12.0  &  H23 (3) &   N/A  \\
Bolo 100  &  03 43 44.0 &  +32 03 10.0  &  250 (14)  &  15.3  &  H26 (3)  &  N/A  \\
Bolo 101  &  03 43 45.6 &  +32 01 45.1  &  139 (19)  &  7.5  &    &   N/A  \\
Bolo 102  &  03 43 50.5 &  +32 03 17.2  &  432 (16)  &  23.5  &  H81 (3) &  N/A  \\
Bolo 103  &  03 43 55.9 &  +32 00 46.4  &  994 (19)  &  56.5  &  \object{HH 211} (13) &  N/A  (IRAS) \\
Bolo 104  &  03 43 57.3 &  +32 03 03.9  &  777 (17)  &  44.2  &  \object[NAME IC 348 MMS]{IC 348-MMS} (14)  &  N/A  \\
Bolo 105  &  03 43 57.8 &  +32 04 06.2  &  283 (16)  &  12.5  &  H17 (3)  &  N/A  \\
Bolo 106  &  03 44 01.6 &  +32 02 02.0  &  426 (18)  &  18.1  &  H16 (3)  &  N/A  \\
Bolo 107  &  03 44 02.1 &  +32 02 33.7  &  388 (18)  &  16.5  &  H18 (3)  &  N/A  \\
Bolo 108  &  03 44 02.3 &  +32 04 57.3  &  139 (16)  &  6.1  &    &   N/A  \\
Bolo 109  &  03 44 05.0 &  +32 00 27.7  &  127 (17)  &  6.3  &    &   N/A  \\
Bolo 110  &  03 44 05.2 &  +32 02 05.6  &  257 (19)  &  11.8  & H20 (3)   &  N/A  \\
Bolo 111  &  03 44 14.5 &  +31 58 00.1  &  170 (17)  &  8.9  &    &   N/A  \\
Bolo 112  &  03 44 14.8 &  +32 09 12.6  &  127 (15)  &  8.2  &    &   N/A  \\
Bolo 113  &  03 44 22.6 &  +31 59 23.2  &  122 (18)  &  6.2  &    &   N/A  \\
Bolo 114  &  03 44 22.7 &  +32 10 01.2  &  140 (15)  &  8.0  &    &   N/A  \\
Bolo 115  &  03 44 36.4 &  +31 58 39.3  &  167 (17)  &  10.4  & H19 (3)  &  N/A  \\
Bolo 116  &  03 44 43.9 &  +32 01 24.6  &  289 (18)  &  18.8  & H14 (3)  &  N/A (IRAS) \\
Bolo 117  &  03 44 48.8 &  +32 00 29.5  &  150 (18)  &  8.7  &  H25 (3) &   N/A  \\
Bolo 118  &  03 44 56.0 &  +32 00 31.3  &  109 (17)  &  5.7  &    &   N/A  \\
Bolo 119  &  03 45 15.9 &  +32 04 48.3  &  181 (16)  &  9.3  &  H90 (3) &   N/A  \\
Bolo 120  &  03 45 48.1 &  +32 24 15.1  &  83 (10)  &  8.8  &  \object[EM* LkHA 330]{LkHA 330}  &  Y   \\
Bolo 121  &  03 47 33.5 &  +32 50 54.9  &  136 (15)  &  6.3  &    &  N   \\
Bolo 122  &  03 47 40.8 &  +32 51 57.2  &  262 (17)  &  14.3  & \object[NAME BARN 5 IRS 1]{B5-IRS1} (15)  &  Y   \\

\enddata

\tablecomments{Numbers in parentheses are $1\sigma$ uncertainties, and do not include an additional systematic uncertainty of 15\% in the peak flux density.  Other names listed are the most common identifications from the literature, and are not meant to be a complete list.  Presence of MIPS source is from the c2d database (Stapelfeldt et al. 2005, in preparation).  References -- (1) \citealt{oling99};  (2) \citealt{bars98}; (3) \citealt{hatch05}; (4) \citealt{froe03}; (5) \citealt{juan93}; (6) \citealt{jenn87}; (7) \citealt{SK01}; (8) \citealt{ladd94}; (9) \citealt{lef98}; (10) \citealt{sand91}; (11) \citealt{bach91}; (12) \citealt{MW02}; (13) \citealt{mcg94}; (14) \citealt{eis03}; (15) \citealt{MA01}.}

\end{deluxetable}

\endinput


==> tab2.tex <==
\ProvidesFile{tab2.tex}
\begin{deluxetable}{lccccccccccl}
\rotate
\tabletypesize{\scriptsize}
\tablecolumns{11}
\tablewidth{0pc}
\tablecaption{Source photometry, masses, column density, sizes, and morphology \label{phottab}}
\tablehead{
\colhead{ID} &  \colhead{Flux($40\arcsec$)}  &  \colhead{Flux($80\arcsec$)}  &  \colhead{Flux($120\arcsec$)} & \colhead{Total Flux}  & \colhead{Mass (10K)}  & \colhead{Peak $A_V$} & \colhead{FWHM} & \colhead{FWHM}  & \colhead{PA} & \colhead{$\mean{n}$}  & \colhead{Morphology\tablenotemark{1}} \\ 
\colhead{} &  \colhead{(Jy)}  &  \colhead{(Jy)}  &  \colhead{(Jy)} & \colhead{(Jy)}  & \colhead{($M_{\sun}$)} & \colhead{(mag)} & \colhead{(minor,$\arcsec$)} & \colhead{(major,$\arcsec$)}  & \colhead{($\degr$)}  &\colhead{(cm$^{-3}$)} & \colhead{}
}
\startdata
Bolo 1  &  \nodata   &   \nodata   &   \nodata    &  0.114 (0.016)  &  0.27 (0.04)       & 8    &  38 (1.1)  &  57 (1.7)  &  -52 (6)  &  1$\times10^5$   &  multiple,round,weak  \\
Bolo 2  &  \nodata   &   \nodata   &   \nodata    &  0.148 (0.016)  &  0.36 (0.04)  	 & 9    &  33 (1.0)  &  54 (1.6)  &  48 (6)  &  3$\times10^5$   &  multiple,round,weak  \\
Bolo 3  &  0.15 (0.02)  &   0.30 (0.05)  &   0.38 (0.07)   &  0.38 (0.07)  &  0.9 (0.2)  & 9    &  65 (1.3)  &  134 (3)  &  -68 (2)  &  3$\times10^4$   &  extended,round,weak  \\
Bolo 4  &  0.21 (0.02)  &   0.48 (0.05)  &   0.87 (0.07)   &  1.24 (0.09)  &  3.0 (0.2)  & 11   &  99 (1.2)  &  122 (1.4)  &  74 (4)  &  5$\times10^4$   &  extended,round  \\
Bolo 5  &  0.93 (0.02)  &   1.48 (0.05)  &   2.05 (0.07)   &  2.05 (0.07)  &  4.9 (0.2)  & 51   &  45 (0.2)  &  79 (0.4)  &  88 (1)  &  7$\times10^5$   &  multiple,extended,elongated  \\
Bolo 6  &  0.19 (0.03)  &   0.43 (0.05)  &   0.79 (0.08)   &  1.18 (0.10)  &  2.9 (0.2)  & 10   &  93 (1.3)  &  132 (1.8)  &  -54 (3)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 7  &  0.16 (0.02)  &   0.36 (0.04)  &   0.67 (0.07)   &  0.96 (0.09)  &  2.3 (0.2)  & 9    &  88 (1.4)  &  122 (1.9)  &  4 (4)  &  4$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 8  &  2.95 (0.03)  &   4.70 (0.05)  &   \nodata    &  4.70 (0.05)  &  11.3 (0.12)   & 160  &  45 (0.1)  &  54 (0.1)  &  -47 (1)  &  4$\times10^6$   &  multiple,extended,round  \\
Bolo 9  &  0.15 (0.02)  &   0.31 (0.04)  &   0.52 (0.07)   &  0.70 (0.09)  &  1.7 (0.2)  & 8    &  76 (1.3)  &  144 (3)  &  -52 (2)  &  3$\times10^4$   &  extended,round,weak  \\
Bolo 10  &  1.22 (0.03)  &   2.04 (0.06)  &   \nodata    &  2.04 (0.06)  &  4.9 (0.14)   & 69   &  53 (0.2)  &  55 (0.2)  &  -10 (10)  &  1$\times10^6$   &  multiple,extended,round  \\
Bolo 11  &  0.31 (0.03)  &   0.75 (0.05)  &   \nodata    &  0.90 (0.06)  &  2.2 (0.15)   & 17   &  78 (0.8)  &  81 (0.8)  &  30 (20)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 12  &  0.16 (0.02)  &   0.37 (0.05)  &   0.69 (0.07)   &  0.97 (0.10)  &  2.3 (0.2) & 8    &  77 (1.2)  &  135 (2)  &  -72 (2)  &  5$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 13  &  \nodata   &   \nodata   &   \nodata    &  0.47 (0.02)  &  1.14 (0.05)  	 & 29   &  44 (0.4)  &  59 (0.5)  &  33 (2)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 14  &  \nodata   &   \nodata   &   \nodata    &  0.41 (0.02)  &  1.00 (0.04)  	 & 24   &  44 (0.4)  &  60 (0.5)  &  -43 (2)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 15  &  0.25 (0.02)  &   \nodata   &   \nodata    &  0.25 (0.02)  &  0.60 (0.06)  	 & 13   &  54 (0.8)  &  60 (0.9)  &  52 (13)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 16  &  0.21 (0.02)  &   \nodata   &   \nodata    &  0.21 (0.02)  &  0.51 (0.06)  	 & 11   &  53 (1.0)  &  58 (1.0)  &  -76 (16)  &  9$\times10^4$   &  multiple,extended,round  \\
Bolo 17  &  0.13 (0.02)  &   0.24 (0.04)  &   0.36 (0.06)   &  0.36 (0.06)  &  0.9 (0.14)& 9    &  67 (1.6)  &  81 (1.9)  &  29 (10)  &  6$\times10^4$   &  extended,round,weak  \\
Bolo 18  &  0.25 (0.02)  &   0.35 (0.04)  &   0.40 (0.06)   &  0.40 (0.06)  &  1.0 (0.15)& 16   &  39 (0.7)  &  45 (0.8)  &  -64 (11)  &  8$\times10^5$   &  extended,round  \\
Bolo 19  &  0.16 (0.02)  &   0.35 (0.04)  &   0.59 (0.06)   &  0.59 (0.06)  &  1.4 (0.14)& 8    &  86 (1.4)  &  93 (1.5)  &  58 (16)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 20  &  0.16 (0.02)  &   0.37 (0.04)  &   0.64 (0.06)   &  0.69 (0.07)  &  1.7 (0.16)& 8    &  75 (1.2)  &  102 (1.7)  &  -82 (4)  &  6$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 21  &  0.22 (0.02)  &   \nodata   &   \nodata    &  0.27 (0.03)  &  0.65 (0.08)  	 & 12   &  44 (0.9)  &  61 (1.2)  &  88 (5)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 22  &  0.41 (0.02)  &   \nodata   &   \nodata    &  0.41 (0.02)  &  0.99 (0.06)  	 & 22   &  44 (0.5)  &  54 (0.6)  &  -66 (4)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 23  &  0.40 (0.02)  &   \nodata   &   \nodata    &  0.40 (0.02)  &  0.96 (0.06)  	 & 20   &  52 (0.5)  &  60 (0.6)  &  75 (5)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 24  &  0.32 (0.03)  &   0.66 (0.05)  &   \nodata    &  0.66 (0.05)  &  1.6 (0.12)   & 16   &  53 (0.6)  &  79 (0.9)  &  -1 (2)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 25  &  0.12 (0.02)  &   0.18 (0.04)  &   0.21 (0.07)   &  0.23 (0.08)  &  0.6 (0.18)& 8    &  51 (1.7)  &  132 (4)  &  -7 (2)  &  2$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 26  &  0.17 (0.02)  &   0.37 (0.04)  &   \nodata    &  0.53 (0.05)  &  1.3 (0.12)   & 8    &  60 (0.9)  &  91 (1.4)  &  -31 (3)  &  8$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 27  &  0.17 (0.02)  &   0.41 (0.04)  &   0.71 (0.06)   &  1.03 (0.09)  &  2.5 (0.2) & 11   &  87 (1.2)  &  136 (1.8)  &  37 (2)  &  4$\times10^4$   &  extended,round  \\
Bolo 28  &  0.15 (0.02)  &   \nodata   &   \nodata    &  0.19 (0.03)  &  0.47 (0.08)  	 & 10   &  36 (0.9)  &  46 (1.2)  &  -66 (8)  &  5$\times10^5$   &  multiple,round  \\
Bolo 29  &  0.35 (0.03)  &   \nodata   &   \nodata    &  0.42 (0.04)  &  1.00 (0.09)  	 & 19   &  33 (0.5)  &  47 (0.7)  &  -53 (4)  &  1$\times10^6$   &  multiple,extended,elongated  \\
Bolo 30  &  0.29 (0.02)  &   \nodata   &   \nodata    &  0.29 (0.02)  &  0.69 (0.05)  	 & 13   &  51 (0.6)  &  56 (0.7)  &  -3 (11)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 31  &  0.59 (0.03)  &   1.24 (0.05)  &   1.92 (0.08)   &  1.92 (0.08)  &  4.6 (0.2) & 27   &  59 (0.4)  &  90 (0.6)  &  -75 (1)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 32  &  0.16 (0.02)  &   0.37 (0.04)  &   0.63 (0.06)   &  0.76 (0.07)  &  1.8 (0.17)& 10   &  94 (1.4)  &  107 (1.6)  &  -68 (9)  &  4$\times10^4$   &  extended,round  \\
Bolo 33  &  0.27 (0.02)  &   \nodata   &   \nodata    &  0.27 (0.02)  &  0.65 (0.05)     & 12   &  55 (0.6)  &  58 (0.6)  &  90 (20)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 34  &  0.19 (0.03)  &   \nodata   &   \nodata    &  0.23 (0.04)  &  0.55 (0.08)  	 & 10   &  40 (1.1)  &  57 (1.6)  &  4 (6)  &  2$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 35  &  0.17 (0.03)  &   \nodata   &   \nodata    &  0.20 (0.04)  &  0.48 (0.08)  	 & 9    &  38 (1.2)  &  56 (1.8)  &  -46 (6)  &  2$\times10^5$   &  multiple,round,weak  \\
Bolo 36  &  0.13 (0.02)  &   0.28 (0.04)  &   0.44 (0.06)   &  0.61 (0.08)  &  1.5 (0.18)& 9    &  65 (1.2)  &  121 (2)  &  72 (2)  &  5$\times10^4$   &  extended,round  \\
Bolo 37  &  0.21 (0.03)  &   0.38 (0.06)  &   \nodata    &  0.38 (0.06)  &  0.9 (0.14)   & 11   &  36 (0.8)  &  75 (1.8)  &  49 (2)  &  2$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 38  &  1.54 (0.03)  &   2.39 (0.06)  &   3.33 (0.08)   &  3.33 (0.08)  &  8.0 (0.2) & 87   &  47 (0.2)  &  63 (0.2)  &  56 (1)  &  2$\times10^6$   &  multiple,extended,elongated  \\
Bolo 39  &  0.29 (0.03)  &   0.59 (0.06)  &   \nodata    &  0.59 (0.06)  &  1.4 (0.14)   & 15   &  42 (0.7)  &  76 (1.2)  &  -32 (2)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo 40  &  0.96 (0.02)  &   \nodata   &   \nodata    &  1.40 (0.03)  &  3.39 (0.08)  	 & 48   &  54 (0.2)  &  63 (0.3)  &  -75 (2)  &  5$\times10^5$   &  multiple,extended,round  \\
Bolo 41  &  0.24 (0.03)  &   0.37 (0.05)  &   \nodata    &  0.37 (0.05)  &  0.9 (0.12)   & 13   &  44 (0.8)  &  63 (1.2)  &  57 (4)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 42  &  1.54 (0.03)  &   \nodata   &   \nodata    &  2.54 (0.04)  &  6.1 (0.10)  	 & 76   &  49 (0.1)  &  56 (0.2)  &  28 (2)  &  2$\times10^6$   &  multiple,extended,round  \\
Bolo 43  &  2.76 (0.03)  &   4.46 (0.06)  &   \nodata    &  4.46 (0.06)  &  10.8 (0.14)  & 150  &  47 (0.1)  &  62 (0.1)  &  59 (1)  &  2$\times10^6$   &  multiple,extended,elongated  \\
Bolo 44  &  0.39 (0.03)  &   0.72 (0.06)  &   \nodata    &  0.72 (0.06)  &  1.7 (0.14)   & 19   &  45 (0.5)  &  78 (0.9)  &  -67 (2)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 45  &  0.68 (0.03)  &   1.35 (0.06)  &   \nodata    &  1.35 (0.06)  &  3.3 (0.14)   & 32   &  55 (0.4)  &  71 (0.5)  &  2 (2)  &  4$\times10^5$   &  multiple,extended,elongated  \\
Bolo 46  &  1.12 (0.03)  &   2.62 (0.06)  &   \nodata    &  2.62 (0.06)  &  6.3 (0.14)   & 52   &  68 (0.2)  &  77 (0.3)  &  41 (2)  &  4$\times10^5$   &  multiple,extended,elongated  \\
Bolo 47  &  0.93 (0.02)  &   2.08 (0.05)  &   \nodata    &  2.81 (0.06)  &  6.8 (0.15)   & 43   &  72 (0.3)  &  85 (0.3)  &  12 (2)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 48  &  6.06 (0.03)  &   9.83 (0.06)  &   \nodata    &  10.59 (0.06)  &  25.6 (0.15) & 370  &  39 (0.0)  &  56 (0.0)  &  -48 (1)  &  1$\times10^7$   &  multiple,extended,round  \\
Bolo 49  &  1.13 (0.03)  &   1.98 (0.06)  &   \nodata    &  1.98 (0.06)  &  4.8 (0.13)   & 59   &  52 (0.2)  &  58 (0.2)  &  -49 (3)  &  1$\times10^6$   &  multiple,extended,elongated  \\
Bolo 50  &  0.45 (0.03)  &   0.96 (0.05)  &   \nodata    &  1.31 (0.07)  &  3.2 (0.16)   & 22   &  68 (0.5)  &  84 (0.6)  &  -39 (3)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 51  &  0.52 (0.03)  &   \nodata   &   \nodata    &  0.62 (0.03)  &  1.49 (0.08)  	 & 30   &  41 (0.3)  &  58 (0.5)  &  -51 (2)  &  5$\times10^5$   &  multiple,extended,round  \\
Bolo 52  &  0.31 (0.02)  &   0.55 (0.05)  &   \nodata    &  0.79 (0.07)  &  1.9 (0.16)   & 19   &  44 (0.5)  &  103 (1.3)  &  89 (1)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 53  &  0.46 (0.03)  &   0.92 (0.05)  &   \nodata    &  1.37 (0.07)  &  3.3 (0.17)   & 24   &  61 (0.5)  &  94 (0.7)  &  13 (1)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 54  &  0.45 (0.03)  &   0.90 (0.05)  &   \nodata    &  1.24 (0.07)  &  3.0 (0.17)   & 23   &  47 (0.4)  &  81 (0.7)  &  72 (1)  &  4$\times10^5$   &  multiple,extended,elongated  \\
Bolo 55  &  0.29 (0.02)  &   \nodata   &   \nodata    &  0.37 (0.03)  &  0.89 (0.07)  	 & 13   &  46 (0.6)  &  59 (0.8)  &  39 (4)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 56  &  0.15 (0.02)  &   0.32 (0.04)  &   0.50 (0.06)   &  0.59 (0.07)  &  1.4 (0.16)& 7    &  78 (1.4)  &  104 (1.9)  &  76 (5)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 57  &  0.30 (0.02)  &   0.51 (0.04)  &   \nodata    &  0.51 (0.04)  &  1.2 (0.10)   & 16   &  42 (0.6)  &  56 (0.7)  &  -80 (4)  &  4$\times10^5$   &  multiple,extended,round  \\
Bolo 58  &  0.26 (0.02)  &   \nodata   &   \nodata    &  0.33 (0.03)  &  0.78 (0.08)  	 & 19   &  39 (0.7)  &  45 (0.8)  &  -47 (10)  &  6$\times10^5$   &  multiple,extended,elongated  \\
Bolo 59  &  0.30 (0.02)  &   0.52 (0.04)  &   \nodata    &  0.52 (0.04)  &  1.24 (0.09)  & 18   &  46 (0.5)  &  56 (0.6)  &  50 (5)  &  3$\times10^5$   &  multiple,extended,elongated  \\
Bolo 60  &  0.16 (0.02)  &   0.28 (0.04)  &   0.37 (0.06)   &  0.37 (0.06)  &  0.9 (0.14)& 9    &  44 (1.0)  &  76 (1.7)  &  -37 (3)  &  1$\times10^5$   &  extended,round,weak  \\
Bolo 61  &  0.12 (0.02)  &   0.22 (0.05)  &   0.37 (0.07)   &  0.37 (0.07)  &  0.9 (0.17)& 8    &  58 (1.7)  &  104 (3)  &  50 (4)  &  5$\times10^4$   &  multiple,round,weak  \\
Bolo 62  &  0.27 (0.02)  &   0.53 (0.05)  &   0.80 (0.07)   &  0.80 (0.07)  &  1.9 (0.17)& 14   &  65 (0.9)  &  80 (1.1)  &  -38 (6)  &  1$\times10^5$   &  multiple,extended,elongated  \\
Bolo 63  &  0.21 (0.02)  &   0.44 (0.04)  &   0.67 (0.06)   &  0.67 (0.06)  &  1.6 (0.13)& 10   &  82 (1.0)  &  89 (1.1)  &  -12 (12)  &  6$\times10^4$   &  extended,elongated  \\
Bolo 64  &  0.11 (0.02)  &   0.17 (0.04)  &   \nodata    &  0.20 (0.05)  &  0.5 (0.12)   & 6    &  37 (1.2)  &  82 (3)  &  53 (3)  &  1$\times10^5$   &  extended,round,weak  \\
Bolo 65  &  0.67 (0.02)  &   \nodata   &   \nodata    &  0.76 (0.03)  &  1.84 (0.07)  	 & 37   &  41 (0.3)  &  48 (0.3)  &  4 (4)  &  1$\times10^6$   &  multiple,extended,elongated  \\
Bolo 66  &  1.32 (0.02)  &   1.83 (0.04)  &   2.31 (0.06)   &  2.31 (0.06)  &  5.6 (0.15)& 76   &  41 (0.1)  &  44 (0.1)  &  -32 (4)  &  4$\times10^6$   &  extended,round  \\
Bolo 67  &  0.23 (0.03)  &   0.45 (0.05)  &   0.70 (0.07)   &  0.86 (0.10)  &  2.1 (0.2) & 12   &  47 (0.7)  &  125 (1.8)  &  37 (1)  &  1$\times10^5$   &  extended,round  \\
Bolo 68  &  0.15 (0.02)  &   0.29 (0.05)  &   \nodata    &  0.36 (0.07)  &  0.9 (0.16)   & 8    &  43 (1.0)  &  95 (2)  &  56 (2)  &  9$\times10^4$   &  extended,round,weak  \\
Bolo 69  &  0.17 (0.02)  &   0.42 (0.04)  &   0.82 (0.07)   &  1.28 (0.09)  &  3.1 (0.2) & 11   &  109 (1.3)  &  128 (1.6)  &  59 (6)  &  4$\times10^4$   &  multiple,extended,round  \\
Bolo 70  &  0.35 (0.02)  &   0.85 (0.05)  &   1.59 (0.07)   &  1.96 (0.08)  &  4.7 (0.2) & 17   &  94 (0.7)  &  112 (0.8)  &  -63 (4)  &  9$\times10^4$   &  multiple,extended,elongated  \\
Bolo 71  &  0.28 (0.03)  &   0.69 (0.05)  &   \nodata    &  1.15 (0.07)  &  2.8 (0.18)   & 13   &  79 (0.8)  &  102 (1.1)  &  61 (3)  &  9$\times10^4$   &  multiple,extended,elongated  \\
Bolo 72  &  0.34 (0.03)  &   0.78 (0.06)  &   \nodata    &  0.93 (0.06)  &  2.2 (0.15)   & 17   &  59 (0.7)  &  84 (1.0)  &  38 (3)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 73  &  0.23 (0.02)  &   0.53 (0.04)  &   0.93 (0.07)   &  1.11 (0.08)  &  2.7 (0.18)& 13   &  87 (1.0)  &  114 (1.3)  &  -79 (3)  &  6$\times10^4$   &  multiple,extended,elongated  \\
Bolo 74  &  0.38 (0.03)  &   \nodata   &   \nodata    &  0.38 (0.03)  &  0.91 (0.07)     & 18   &  51 (0.6)  &  60 (0.7)  &  52 (6)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 75  &  0.38 (0.03)  &   \nodata   &   \nodata    &  0.38 (0.03)  &  0.91 (0.07)  	 & 18   &  51 (0.6)  &  61 (0.7)  &  -54 (6)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 76  &  0.16 (0.02)  &   0.32 (0.04)  &   \nodata    &  0.43 (0.05)  &  1.0 (0.13)   & 8    &  64 (1.2)  &  89 (1.7)  &  89 (5)  &  6$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 77  &  0.13 (0.03)  &   0.24 (0.05)  &   0.38 (0.08)   &  0.38 (0.08)  &  0.9 (0.18)& 8    &  72 (2)  &  97 (3)  &  -62 (8)  &  4$\times10^4$   &  multiple,round,weak  \\
Bolo 78  &  0.36 (0.02)  &   0.72 (0.04)  &   \nodata    &  0.93 (0.05)  &  2.3 (0.13)   & 19   &  65 (0.6)  &  77 (0.7)  &  -78 (4)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo 79  &  0.98 (0.03)  &   \nodata   &   \nodata    &  1.84 (0.04)  &  4.4 (0.11)  	 & 43   &  59 (0.2)  &  64 (0.3)  &  4 (4)  &  6$\times10^5$   &  multiple,extended,round  \\
Bolo 80  &  1.36 (0.03)  &   2.26 (0.06)  &   \nodata    &  3.08 (0.08)  &  7.4 (0.18)   & 77   &  57 (0.2)  &  76 (0.3)  &  -62 (1)  &  7$\times10^5$   &  multiple,extended,elongated  \\
Bolo 81  &  1.62 (0.03)  &   \nodata   &   \nodata    &  2.61 (0.05)  &  6.3 (0.12)  	 & 86   &  53 (0.2)  &  59 (0.2)  &  -26 (2)  &  1$\times10^6$   &  multiple,extended,round  \\
Bolo 82  &  0.20 (0.02)  &   \nodata   &   \nodata    &  0.36 (0.04)  &  0.88 (0.09)  	 & 10   &  54 (1.0)  &  62 (1.2)  &  -4 (11)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 83  &  0.21 (0.02)  &   0.47 (0.05)  &   \nodata    &  0.47 (0.05)  &  1.1 (0.11)   & 12   &  60 (1.0)  &  74 (1.2)  &  75 (6)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 84  &  0.25 (0.03)  &   \nodata   &   \nodata    &  0.47 (0.05)  &  1.1 (0.12)  	 & 13   &  61 (0.9)  &  68 (1.0)  &  21 (11)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 85  &  0.19 (0.02)  &   0.40 (0.05)  &   \nodata    &  0.40 (0.05)  &  1.0 (0.11)   & 11   &  54 (1.0)  &  77 (1.4)  &  72 (4)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 86  &  0.13 (0.02)  &   0.27 (0.05)  &   0.43 (0.07)   &  0.64 (0.10)  &  1.5 (0.2) & 9    &  80 (1.7)  &  132 (3)  &  -39 (3)  &  3$\times10^4$   &  extended,round,weak  \\
Bolo 87  &  0.13 (0.02)  &   0.25 (0.04)  &   0.41 (0.06)   &  0.45 (0.07)  &  1.1 (0.16)& 7    &  68 (1.5)  &  101 (2)  &  70 (4)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 88  &  0.21 (0.02)  &   0.52 (0.04)  &   0.97 (0.07)   &  1.43 (0.09)  &  3.4 (0.2) & 11   &  94 (1.0)  &  152 (1.6)  &  -39 (2)  &  4$\times10^4$   &  extended,elongated  \\
Bolo 89  &  0.19 (0.02)  &   0.44 (0.04)  &   0.74 (0.06)   &  0.99 (0.08)  &  2.4 (0.2) & 11   &  81 (1.0)  &  126 (1.6)  &  -17 (2)  &  5$\times10^4$   &  extended,round  \\
Bolo 90  &  \nodata   &   \nodata   &   \nodata    &  0.126 (0.015)  &  0.31 (0.04)  	 & 10   &  22 (0.9)  &  33 (1.2)  &  -90 (8)  &  \nodata   &  extended,round  \\
Bolo 91  &  0.14 (0.02)  &   0.24 (0.04)  &   0.35 (0.06)   &  0.37 (0.07)  &  0.9 (0.17)& 8    &  58 (1.5)  &  105 (3)  &  -79 (3)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 92  &  0.13 (0.02)  &   0.24 (0.04)  &   \nodata    &  0.24 (0.04)  &  0.57 (0.09)  & 7    &  54 (1.4)  &  67 (1.7)  &  56 (10)  &  8$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 93  &  0.17 (0.02)  &   0.38 (0.04)  &   0.66 (0.06)   &  0.89 (0.08)  &  2.2 (0.2) & 8    &  92 (1.4)  &  111 (1.7)  &  33 (6)  &  4$\times10^4$   &  extended,round,weak  \\
Bolo 94  &  0.16 (0.02)  &   0.32 (0.04)  &   \nodata    &  0.32 (0.04)  &  0.77 (0.09)  & 9    &  57 (1.2)  &  67 (1.3)  &  66 (10)  &  9$\times10^4$   &  multiple,extended,round  \\
Bolo 95  &  0.14 (0.02)  &   0.28 (0.04)  &   0.51 (0.06)   &  0.77 (0.08)  &  1.9 (0.18)& 8    &  93 (1.4)  &  116 (1.8)  &  27 (6)  &  3$\times10^4$   &  extended,round,weak  \\
Bolo 96  &  0.22 (0.02)  &   \nodata   &   \nodata    &  0.46 (0.04)  &  1.1 (0.09)      & 10   &  59 (0.8)  &  70 (1.0)  &  8 (6)  &  1$\times10^5$   &  multiple,extended,round  \\
Bolo 97  &  0.22 (0.02)  &   \nodata   &   \nodata    &  0.35 (0.03)  &  0.85 (0.08)  	 & 11   &  60 (0.9)  &  66 (1.0)  &  -40 (15)  &  1$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 98  &  0.20 (0.02)  &   \nodata   &   \nodata    &  0.32 (0.04)  &  0.77 (0.09)  	 & 9    &  59 (1.0)  &  64 (1.1)  &  89 (16)  &  9$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 99  &  0.24 (0.02)  &   \nodata   &   \nodata    &  0.43 (0.03)  &  1.04 (0.07)  	 & 12   &  53 (0.6)  &  61 (0.7)  &  75 (6)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo 100  &  0.41 (0.02)  &   \nodata   &   \nodata    &  0.81 (0.03)  &  1.95 (0.08)  	 & 18   &  59 (0.4)  &  67 (0.5)  &  -7 (5)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo 101  &  0.21 (0.03)  &   \nodata   &   \nodata    &  0.35 (0.04)  &  0.8 (0.10)  	 & 10   &  48 (0.9)  &  66 (1.3)  &  49 (5)  &  1$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 102  &  0.63 (0.02)  &   1.41 (0.04)  &   \nodata    &  1.41 (0.04)  &  3.4 (0.11)  & 31   &  62 (0.3)  &  76 (0.4)  &  7 (2)  &  3$\times10^5$   &  multiple,extended,round  \\
Bolo 103  &  1.28 (0.03)  &   2.07 (0.05)  &   \nodata    &  2.42 (0.06)  &  5.8 (0.15)  & 70   &  46 (0.2)  &  57 (0.2)  &  49 (1)  &  2$\times10^6$   &  multiple,extended,elongated  \\
Bolo 104  &  1.05 (0.02)  &   \nodata   &   \nodata    &  1.42 (0.03)  &  3.43 (0.08)  	 & 55   &  46 (0.2)  &  55 (0.2)  &  77 (2)  &  1$\times10^6$   &  multiple,extended,round  \\
Bolo 105  &  0.40 (0.02)  &   \nodata   &   \nodata    &  0.61 (0.03)  &  1.47 (0.08)  	 & 20   &  51 (0.4)  &  64 (0.5)  &  -7 (3)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 106  &  \nodata   &   \nodata   &   \nodata    &  0.50 (0.02)  &  1.21 (0.04)  	 & 30   &  52 (0.4)  &  55 (0.4)  &  -87 (10)  &  3$\times10^5$   &  multiple,extended,round  \\
Bolo 107  &  \nodata   &   \nodata   &   \nodata    &  0.48 (0.02)  &  1.17 (0.04)  	 & 27   &  53 (0.3)  &  60 (0.4)  &  -76 (4)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo 108  &  0.18 (0.02)  &   \nodata   &   \nodata    &  0.32 (0.04)  &  0.78 (0.09)  	 & 10   &  53 (0.9)  &  72 (1.2)  &  -59 (5)  &  9$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 109  &  0.16 (0.02)  &   0.33 (0.05)  &   \nodata    &  0.39 (0.05)  &  0.9 (0.13)  & 9    &  50 (1.1)  &  80 (1.8)  &  61 (4)  &  1$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 110  &  0.44 (0.03)  &   \nodata   &   \nodata    &  0.44 (0.03)  &  1.05 (0.06)  	 & 18   &  53 (0.5)  &  59 (0.5)  &  89 (7)  &  2$\times10^5$   &  multiple,extended,elongated  \\
Bolo 111  &  0.22 (0.02)  &   0.47 (0.04)  &   0.71 (0.07)   &  0.83 (0.08) &  2.0 (0.19)& 12   &  71 (1.0)  &  101 (1.5)  &  -45 (3)  &  8$\times10^4$   &  multiple,extended,round  \\
Bolo 112  &  0.17 (0.02)  &   0.33 (0.04)  &   \nodata    &  0.45 (0.06)  &  1.1 (0.14)  & 9    &  60 (1.3)  &  65 (1.3)  &  -70 (20)  &  1$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 113  &  0.18 (0.02)  &   0.35 (0.05)  &   0.56 (0.07)   &  0.74 (0.09)  &  1.8 (0.2)& 9    &  75 (1.3)  &  112 (2)  &  9 (3)  &  5$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 114  &  0.18 (0.02)  &   0.38 (0.04)  &   \nodata    &  0.55 (0.05)  &  1.3 (0.13)  & 10   &  59 (1.0)  &  88 (1.4)  &  -53 (3)  &  9$\times10^4$   &  multiple,extended,elongated  \\
Bolo 115  &  0.22 (0.02)  &   0.37 (0.05)  &   0.53 (0.07)   &  0.54 (0.08) &  1.3 (0.19)& 12   &  45 (0.8)  &  96 (1.8)  &  -39 (2)  &  1$\times10^5$   &  extended,elongated  \\
Bolo 116  &  0.39 (0.02)  &   0.51 (0.05)  &   \nodata    &  0.51 (0.05)  &  1.2 (0.12)  & 20   &  35 (0.5)  &  47 (0.6)  &  46 (4)  &  1$\times10^6$   &  multiple,extended,round  \\
Bolo 117  &  0.22 (0.02)  &   0.40 (0.05)  &   \nodata    &  0.40 (0.05)  &  1.0 (0.11)  & 11   &  44 (0.8)  &  70 (1.3)  &  76 (3)  &  2$\times10^5$   &  multiple,extended,round,weak  \\
Bolo 118  &  0.14 (0.02)  &   0.29 (0.05)  &   \nodata    &  0.34 (0.05)  &  0.8 (0.12)  & 8    &  47 (1.1)  &  88 (2)  &  4 (3)  &  9$\times10^4$   &  multiple,extended,round,weak  \\
Bolo 119  &  0.24 (0.02)  &   0.53 (0.04)  &   0.91 (0.06)   &  1.29 (0.09)  &  3.1 (0.2)& 13   &  92 (1.0)  &  123 (1.4)  &  -89 (3)  &  5$\times10^4$   &  extended,elongated  \\
Bolo 120  &  \nodata   &   \nodata   &   \nodata    &  0.08 (0.01)  &  0.19 (0.02)       & 6    &  24 (0.9)  &  25 (1.0)  &  -3 (90)  &  \nodata   &  multiple,extended,round,weak  \\
Bolo 121  &  0.18 (0.02)  &   0.44 (0.04)  &   \nodata    &  0.65 (0.05)  &  1.6 (0.12)  & 10   &  85 (1.1)  &  94 (1.2)  &  -86 (11)  &  5$\times10^4$   &  multiple,extended,elongated  \\
Bolo 122  &  0.38 (0.02)  &   0.88 (0.04)  &   \nodata    &  1.34 (0.06)  &  3.2 (0.15)  & 19   &  63 (0.5)  &  91 (0.7)  &  -63 (2)  &  2$\times10^5$   &  multiple,extended,elongated  \\
\enddata
\tablecomments{Masses are calculated according to Equation~\ref{masseq} from the total flux density assuming a single dust temperature of $T_D=10K$ and a dust opacity at 1.1mm of $\kappa_{1.1mm} = 0.0114$~cm$^2$g$^{-1}$.  Peak $A_V$ is calculated from the peak flux density as in Section~\ref{avsect}.  FWHM and PAs are from a gaussian fit; the PA is measured in degrees east of north of the major axis.  $\mean{n}$ is the mean particle density as calculated from the total mass and the deconvolved average FWHM size.  Numbers in parentheses are $1\sigma$ uncertainties.  Uncertainties for masses are from photometry only, and do not include uncertainties from $\kappa$, $T_D$, or $d$, which can be up to a factor of a few or more.  Uncertainties for the FWHM and PA are formal fitting errors from the elliptical gaussian fit; additional uncertainties of $10-15$\% apply to the FWHM, and $\sim5\degr$ to the PA (determined from simulations).}
\tablenotetext{1}{The morphology keyword(s) given indicates whether the source is multiple (within $3\arcmin$ of another source), extended (major axis FW at $2\sigma > 1\arcmin$), elongated (axis ratio at $4\sigma > 1.2$), round (axis ratio at $4\sigma < 1.2$), or weak (peak flux densities less than 5 times the RMS/pixel in the unfiltered map).}
\end{deluxetable}
\endinput

